Partition genericity and pigeonhole basis theorems

There exist two notions of typicality in computability theory, namely, genericity and randomness. In this article, we introduce a new notion of genericity, called partition genericity, which is at the intersection of these two notions of typicality, and show that many basis theorems apply to partition genericity. More precisely, we prove that every co-hyperimmune set and every Kurtz random is partition generic, and that every partition generic set admits weak infinite subsets. In particular, we answer a question of Kjos-Hanssen and Liu by showing that every Kurtz random admits an infinite subset which does not compute any set of positive Hausdorff dimension. Partition genericty is a partition regular notion, so these results imply many existing pigeonhole basis theorems.

==> parts/part6-cb-traces.tex <==

\ludovic{TODO, there is something wrong in this section.}

The purpose of this section is to find the right genericity notion admitting an avoidance of constant-bound traces for arbitrary closed classes in the Cantor space. The following theorem was proven by Liu~\cite{liu2015cone}:

\begin{theorem}[Liu~\cite{liu2015cone}]\label[theorem]{thm:avoidance-closed-pigeon-basis}
If $\C \subseteq 2^\omega$ is a closed class with no computable c.b-trace, then for every set $A \subseteq \omega$, there is an infinite set $H \subseteq A$ or $H \subseteq \overline{A}$ such that $\C$ has no $H$-computable c.b-trace.
\end{theorem}

This theorem for Liu was proven to separate Ramsey's theorem for pairs from weak weak K\"onig's lemma in reverse mathematics. Such a separation is already witnessed by a $\Pi^0_1$ class with no computable c.b-trace, namely, any class with only Martin-L\"of randoms. Then, the separation already follows from \Cref{cor:liu-effective-closed-sets}. In this section, we try to extend \Cref{thm:theorem-partition-generic-trace} to non-effectively closed classes.

Here again, partition genericity is not the right notion to reprove this pigeonhole basis theorem. Indeed, the following proposition shows that there is no avoidance of constant-bound traces  partition genericity basis theorem.

\begin{proposition}\label[proposition]{prop:pg-non-basis-avoidance-cbtraces}
There is a closed class~$\C \subseteq 2^\omega$ with no computable c.b-trace, and a partition generic set~$A$ such that every infinite subset of~$A$ computes a c.b-trace of~$\C$.
\end{proposition}
\begin{proof}
\ludovic{TODO}
\end{proof}

The remainder of this section is devoted to the design of a notion of genericity which admits an avoidance of constant-bound traces basis theorem, implying \Cref{thm:avoidance-closed-pigeon-basis}.

\subsection{Trace genericity}

From now on, fix a closed class~$\C \subseteq 2^\omega$ with no computable c.b-trace. All the following definitions hold for any closed class~$\C$, but because of~\Cref{lem:comb-trace-theorem}, the only interesting case is when the class~$\C$ has no computable c.b-trace. For every~$n \in \omega$, let $C_n \subseteq 2^{=n}$ be the (finite) set of strings~$\sigma$ of length~$n$ such that $[\sigma] \cap \C \neq \emptyset$. 

In the following, we identify a finite set of strings~$V \subseteq 2^{<\omega}$ to its corresponding clopen class in the Cantor space $[V] = \{ X \in 2^\omega : \exists \sigma \in V : \sigma \prec X \}$. Note that if~$V_0, V_1 \subseteq 2^{=n}$ are two sets, then $V_0 \cap V_1 \neq \emptyset$ iff $[V_0] \cap [V_1] \neq \emptyset$. This property fails when the length of the strings in~$V_0$ and $V_1$ differ.

\begin{definition}
A sequence of $m$ clopen sets $V_0, \dots, V_{m-1} \subseteq 2^{=n}$
	is \emph{$k$-disperse} if for every $k$-cover
	$(P_j : j < k)$ of $\{0, \dots, m-1\}$, there exists a $j < k$
	such that $\bigcap_{s \in P_\nu} [V_s] = \emptyset$.
\end{definition}


\begin{definition}
A class $\A \subseteq 2^\omega \times \P(2^{<\omega})$ is \emph{$\mathfrak{T}(\C)$-large} if
\begin{enumerate}
\item If $(X,V) \in \A$ and $X \subseteq Y$, then $(Y,V) \in \A$
\item For every~$n \in \omega$, every sequence of clopen sets $V_0, \dots, V_{m-1} \subseteq 2^{=n}$ such that $\bigcap_{s < m} [V_s] = \emptyset$, and every~$k \in \omega$, there is some~$s < m$ such that for every $k$-cover $Y_0, \dots, Y_{k-1}$ of $\omega$, there is some~$j < k$ such that  $(Y_j, V_s) \in \A$.
\end{enumerate}
\end{definition}

%The definition of $\mathfrak{T}(\C)$-largeness ensures that for every~$n \in B$, the class $\{ X : (X,n) \in \A \}$ is partition large. 
As for enumeration genericity, if $\C$ admits no computable c.b-trace but $\A$ is $\Sigma^0_1$, then there must be some \qt{overflow}, in the following sense.

\begin{lemma}[Liu~\cite{liu2015cone}]\label[lemma]{lem:comb-trace-theorem}
Suppose $\C$ has no computable c.b-trace. For every c.e.\ set of clopen sets $E$, 
one of the following must hold:
\begin{enumerate}
	\item $C_n \in E$ for some~$n \in \omega$;
	\item For every~$k$, there is some~$n$ and a $k$-disperse sequence of clopen sets $V_0, \dots, V_{m-1} \subseteq 2^{=n}$ disjoint from $E$.
\end{enumerate}
\end{lemma}
%\begin{proof}
%\ludovic{TODO, give the general proof}
%%Define the following $D$-c.e. set.
%%$$
%%E = \{ W \in \W : (\forall \rho, \sigma \in W)|\rho| = |\sigma| \wedge  \varphi(W) \}
%%$$
%Suppose case 1 does not hold. In other words $C_n \not \in E$ for every $n \in \omega$.
%For every~$n$, let 
%$$
%\W_n = \{ V \subseteq 2^{=n} : V \not \in E\}
%$$
%We prove that for almost every $n \in \omega$, $\bigcap_{V \in \W_n} [V] = \emptyset$.
%Note that $\W_n$ is co-c.e.\ uniformly in $n$, and by assumption, $C_n \in \W_n$.
%
%Let~$n$ be such that $\bigcap_{V \in \W_n} [V] \neq \emptyset$.
%Since all the strings in the clopen sets have the same length, there is some~$\rho \in \bigcap_{V \in \W_n} V$.
%Moreover, since $C_n \in \W_n$, then for any such~$\rho$, $[\rho] \cap \C \neq \emptyset$.
%
%Thus, if there are infinitely many~$n$ such that $\bigcap_{V \in \W_n} [V] \neq \emptyset$,
%we can find these computably, and create a c.b-trace of~$\C$, contradicting our assumption.
%%
%%
%%Therefore if  there exists a $k$-cover $(P_\nu : \nu < k)$
%%of $\W_n$ such that $(\forall \nu < k)\bigcap_{W \in P_\nu} W \neq \emptyset$, then this cover
%%can be found in a finite amount of time. Furthermore $C_n \in P_\nu$ for some $\nu < k$,
%%so 
%%$$
%%(\forall \rho \in \bigcap_{W \in P_\nu} W) [\rho] \cap \C \neq \emptyset
%%$$
%%It follows that if there exists infinitely many $n$ such that such a $k$-cover exists,
%%we can computably find infinitely of them and define the computable enumeration $h$
%%which on input $n$ returns $(\rho_\nu : \nu < k)$ such that there exists some $t, m \geq n$ 
%%and a $k$-cover $(P_\nu : \nu < k)$ of $\W_{m, t}$ such that
%%$(\forall \nu < k)\bigcap_{W \in P_\nu} W \neq \emptyset$
%%and $\rho_\nu$ is the leftmost string in $\bigcap_{W \in P_\nu} W$.
%%This contradicts the fact that  $\C$ has no computable c.b-trace.
%\end{proof}

\begin{proposition}\label[proposition]{prop:prtrace-pg-large-ce}
Suppose $\C$ has no computable c.b-trace.
For every non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class~$\U \subseteq 2^\omega \times \P(2^{<\omega})$, the class $\{ X : \exists n\ (X, C_n) \in \U \}$ is partition large.
\end{proposition}
\begin{proof}
Suppose $\C$ has no computable c.b-trace. Let $\U \subseteq 2^\omega \times \P(2^{<\omega})$ be any non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class. Let~$A_k = \{ V : \forall Z_0, \dots, Z_{k-1} \exists i < k\ (Z_i, V) \in \U \}$.
The set~$A_k$ is c.e. Moreover, for every~$n \in \omega$ and every finite sequence of clopen sets $V_0, \dots, V_{m-1} \subseteq 2^{=n}$ such that $\bigcap_{s < m} [V_s] = \emptyset$, there is some~$s < m$ such that~$V_s \in A_k$. By~\Cref{lem:comb-trace-theorem}, $C_n \in A_k$ for some~$n \in \omega$.
Thus the class~$\{ X : \exists n\ (X, C_n) \in \U \}$ is partition large.
\end{proof}


%\begin{definition}
%A class $\A \subseteq 2^\omega \times \P(2^{<\omega})$ is \emph{$\mathfrak{T}(\C)$-large} if
%\begin{enumerate}
%\item For every~$n \in B$, $(\omega, n) \in \A$;
%\item If $(X,n) \in \A$ and $X \subseteq Y$, then $(Y,n) \in \A$
%\item If $(\omega, n) \in \A$, then for every $k$-cover $Y_0, \dots, Y_{k-1}$ of $\omega$, there is some $j < k$ such that $(Y_j, n) \in \A$.
%\end{enumerate}
%\end{definition}

A class~$\A \subseteq 2^\omega \times \P(2^{<\omega})$ is \emph{non-trivial} if for every~$(X,V) \in \A$, $|X| \geq 2$. 

\begin{definition}
Let $\A \subseteq 2^\omega \times \P(2^{<\omega})$ be a class.
We say that $X$ is \emph{$\mathfrak{T}(\C)$-generic} in $\A$ if for every non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class~$\U \subseteq \A$, $X \in \L(\{ Z : \exists n\ (Z, C_n) \in \U \})$. If $X$ is $\mathfrak{T}(\C)$-generic in $2^\omega \times  \P(2^{<\omega})$, we simply say that $X$ is \emph{$\mathfrak{T}(\C)$-generic}.
\end{definition}


\begin{proposition}\label[proposition]{prop:nocb-and-pg-rel-then-prtrace-gen}
Suppose $\C$ has no computable c.b-trace and $A$ is partition generic relative to~$\C$.
Then $A$ is $\mathfrak{T}(\C)$-generic.
\end{proposition}
\begin{proof}
Fix a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class~$\U \subseteq 2^\omega \times \P(2^{<\omega})$.
Since~ $\C$ has no computable c.b-trace, by \Cref{prop:prtrace-pg-large-ce}, the class $\V = \{ X : \exists n\ (X, C_n) \in \U \}$ is partition large. Note that $\V$ is $\Sigma^0_1(\C)$.
By \Cref{prop:large-contains-pr}, $\V$ contains a partition regular subclass, so $\L(\V)$ is partition regular. By \Cref{prop:complarge}, $\L(\V)$ is $\Pi^0_2(\C)$, so since $A$ is partition generic relative to~$\C$, $A \in \L(\V)$.
\end{proof}


\begin{proposition}\label[proposition]{prop:prtrace-pg-omega-ce}
Suppose $\C$ has no computable c.b-trace. Then $\omega$ is $\mathfrak{T}(\C)$-generic.	
\end{proposition}
\begin{proof}
Immediate from \Cref{prop:nocb-and-pg-rel-then-prtrace-gen}, since $\omega$ is partition generic relative to~$\C$.
%
%Fix a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class~$\U \subseteq 2^\omega \times \P(2^{<\omega})$.
%Since~$B$ is not c.e., by \Cref{prop:prtrace-pg-large-ce}, the class $\V = \{ X : \exists n \in \overline{B}\ (X, n) \in \U \}$ is partition large.
%By \Cref{prop:large-contains-pr}, $\V$ contains a partition regular subclass, so $\L(\V)$ is partition regular. In particular, $\omega \in \L(\V)$. 
\end{proof}

\begin{proposition}\label[proposition]{prop:prtrace-pg-infinite}
If $X$ is $\mathfrak{T}(\C)$-generic in a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class $\A \subseteq 2^\omega \times \P(2^{<\omega})$, then $X$ is infinite.
\end{proposition}
\begin{proof}
Let~$\V = \{ Z : \exists n\ (Z, C_n) \in \A \}$. Since $X$ is $\mathfrak{T}(\C)$-generic in~$\A$, $X \in \L(\V)$. Since $\A$ is non-trivial, for every~$X \in \V$, $|X| \geq 2$. Therefore, by \Cref{prop:non-trivial-u2}, $\L(\V)$ is non-trivial, so since~$X \in \L(\V)$, $X$ is infinite.
\end{proof}

\begin{proposition}\label[proposition]{prop:prtrace-pg-invariant-superset}
If $X$ is $\mathfrak{T}(\C)$-generic in $\A$	 and $Y \supseteq X$, then $Y$ is $\mathfrak{T}(\C)$-generic in~$\A$.
\end{proposition}
\begin{proof}
Let $\U$ be a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ subclass of~$\A$. Since $X$ is $\mathfrak{T}(\C)$-generic in $\A$, then, letting~$\V = \{ Z : \exists n\ (Z, C_n) \in \U \}$, $X \in \L(\V)$. Since $\L(\V)$ is closed upward, $Y \in \L(\V)$.
Therefore $Y$ is $\mathfrak{T}(\C)$-generic in~$\A$.
\end{proof}

\begin{proposition}\label[proposition]{prop:prtrace-pg-invariant-finite}
If $X$ is $\mathfrak{T}(\C)$-generic in $\A$ and $Y =^{*} X$, then $Y$ is $\mathfrak{T}(\C)$-generic in~$\A$.
\end{proposition}
\begin{proof}
Let $\U \subseteq \A$ be any non-trivial $\mathfrak{T}(\C)$-large  $\Sigma^0_1$ subclass of $\A$.
Let~$\V = \{ Z : \exists n\ (Z, C_n) \in \U \}$. Since $X$ is $\mathfrak{T}(\C)$-generic in $\A$, then $X \in \L(\V)$. 
Since $Y =^{*} X$, then there is a finite set $F$ such that $Y \cup F \supseteq X$.
By partition regularity of~$\L(\V)$, either $F \in \L(\V)$, or $Y \in \L(\V)$. 
Since~$\U$ is non-trivial, then $\L(\V)$ is non-trivial, so $F \not \in \L(\V)$. It follows that $Y \in \L(\V)$.
Therefore $Y$ is $\mathfrak{T}(\C)$-generic in~$\A$.
\end{proof}

\begin{lemma} \label{lemma:prtrace-abslarge2}
Suppose $X$ is $\mathfrak{T}(\C)$-generic in a class~$\A \subseteq 2^\omega \times \P(2^{<\omega})$. For every $Y_0 \cup Y_1 \supseteq X$, if $Y_0 \not \in \L(\{ Z : \exists n \ (Z, C_n) \in \A \})$, then $Y_1$ is $\mathfrak{T}(\C)$-generic in~$\A$.
\end{lemma}
\begin{proof}
Fix any non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class $\U \subseteq \A$ and let~$\V = \{ Z : \exists n\ (Z, C_n) \in \U \}$. 
Since $X$ is $\mathfrak{T}(\C)$-generic in~$\A$, then $X \in \L(\V)$. Since $Y_0 \cup Y_1 \supseteq X$, then by partition regularity of $\L(\V)$, either~$Y_0 \in \L(\V)$, or $Y_1 \in \L(\V)$. Since~$\U \subseteq \A$, then $\V \subseteq \{ Z : \exists n\ (Z, C_n) \in \A \}$, so $\L(\V) \subseteq \L(\{ Z : \exists n\ (Z, C_n) \in \A \})$. If follows from hypothesis that~$Y_0 \not \in \L(\V)$, so $Y_1 \in \L(\V)$.
Therefore, $Y_1$ is $\mathfrak{T}(\C)$-generic in~$\A$.
\end{proof}

\begin{proposition} \label[proposition]{lemma:prtrace-abslarge}
Let $\A \subseteq 2^\omega \times \P(2^{<\omega})$ be a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class. Suppose $X$ is $\mathfrak{T}(\C)$-generic in $\A$. Let $Y_0 \cup \dots \cup Y_k \supseteq X$. Then there is a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ subclass $\U \subseteq \A$ together with some $i \leq k$ such that $Y_i$ is $\mathfrak{T}(\C)$-generic in $\U$.
\end{proposition}
\begin{proof}
We proceed by induction on $k$. For $k = 0$, $Y_0 \supseteq X$, so by \Cref{prop:prtrace-pg-invariant-superset}, $Y$ is $\mathfrak{T}(\C)$-generic in $\A$. Take $\U = \A$ and we are done.
Suppose now that the property holds for $k-1$. Suppose $Y_k$ is not $\mathfrak{T}(\C)$-generic in $\A$. 
Thus there is a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class $\U \subseteq \A$ such that $Y_k \not\in \L(\{ Z : \exists n\ (Z, C_n) \in \U \})$.
By \Cref{lemma:prtrace-abslarge2}, $Y_0 \cup \dots \cup Y_{k-1}$ is $\mathfrak{T}(\C)$-generic in $\U$. By induction hypothesis on $\U$ and $Y_0 \cup \dots \cup Y_{k-1}$, there is a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ subclass $\V \subseteq \U$ together with some $i < k$ such that $Y_i$ is $\mathfrak{T}(\C)$-generic in $\V$.
\end{proof}


\subsection{Applications}

We now turn to the main application of trace genericity, which is a partition genericity subset basis theorem for avoidance of constant-bound traces of closed classes.

\begin{theorem}\label[theorem]{thm:pg-traceg-ce}
Suppose~$A$ is $\mathfrak{T}(\C)$-generic in a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class~$\U \subseteq 2^\omega \times \P(2^{<\omega})$.
Then there is an infinite subset $H \subseteq A$ such that~$\C$ has no $H$-computable c.b-trace.
\end{theorem}
\begin{proof}
Consider the notion of forcing $(\sigma, X, \V)$ where $(\sigma, X)$ is as Mathias condition, 
and $\V \subseteq \U$ is a $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class within which $X$ is $\mathfrak{T}(\C)$-generic.
A condition $(\tau, Y, \W)$ \emph{extends} another condition $(\sigma, X, \V)$ if $(\tau, Y)$ Mathias extends $(\sigma, X)$ and $\W \subseteq \V$.

Any filter $\F$ induce a subset $G_\F = \bigcup_{(\sigma, X, \V) \in \F} \sigma$ of~$A$. 
The first property we prove is that $G_\F$ is an infinite set. % $A$ is partition generic and $\F$ is a sufficiently generic filter containing $(\emptyset, A, 2^\omega)$, then $G_\F$ is a partition generic subset of $A$. In particular, $G_\F$ is an infinite set.

\begin{lemma}\label[lemma]{lem:pg-traceg-forcing-infinite}
Let $\F$ be a sufficiently generic filter. Then $G_\F$ is infinite.
\end{lemma}
\begin{proof}
Let us show that for any $n$, the set of conditions $(\tau, Y, \V)$ such that $\tau(x) = 1$ for some $x > n$ is dense.
Let $(\sigma, X, \V)$ be a condition. Since $X$ is $\mathfrak{T}(\C)$-generic in $\V$, then by \Cref{prop:prtrace-pg-infinite}, $X$ is infinite. Let $x \in X$ be greater than $n$, let $\tau$ be string $\sigma \cup \{x\}$ and let $Y = X \setminus \{0, \dots, |\rho|\}$. By \Cref{prop:prtrace-pg-invariant-finite}, $Y$ is $\mathfrak{T}(\C)$-generic in $\V$. Therefore, $(\tau, Y, \V)$ is a valid extension of $(\sigma, X, \V)$.
\end{proof}

In what follows, we assume that $\Phi_e$ is a c.b-trace functional, in the sense that for every oracle~$X$, if~$\Phi^X_e(n)\downarrow$, then $\Phi^X_e(n)$ is a binary string of length~$n$.

\begin{lemma}\label[lemma]{lem:pg-traceg-forcing-requirement}
For every condition $(\sigma, X, \V)$, there is an extension $(\tau, Y, \W)$ forcing $\Phi_e^G$ not to be a c.b-trace of~$\C$.	
\end{lemma}
\begin{proof}
We have two cases.

Case 1: the following class is $\mathfrak{T}(\C)$-large:
$$
\A = \{ (Y,V) \in \V : \exists \rho \subseteq Y\ \exists n\ V \subseteq 2^{=n} \wedge \in [\Phi_e^{\sigma \cup \rho}(n)] \cap [V] = \emptyset \}
$$
Since $\A$ is a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ subclass of~$\U$ and $X$ is $\mathfrak{T}(\C)$-generic in~$\U$, then $X \in \L(\{ Z : \exists n\ (Z,C_n) \in \A \})$. In particular, $(X, C_n) \in \A$ for some~$n$. Therefore there is some~$\rho \subseteq X$ and some~$n$ such that $\Phi_e^{\sigma \cup \rho}(n)\downarrow = \mu$ for some string~$\mu$ of length~$n$ such that~$[\mu] \cap [C_n] = \emptyset$. By definition of~$C_n$, then $[U] \cap \C = \emptyset$. Let~$Y = X \setminus \{0, \dots, |\rho|\}$. By \Cref{prop:prtrace-pg-invariant-finite}, $Y$ is $\mathfrak{T}(\C)$-generic in~$\V$. Therefore $(\sigma \cup \rho, Y, \V)$ is an extension of~$(\sigma, X, \V)$ forcing $\Phi_e^G$ not to be a c.b-trace of~$\C$.

Case 2: there is some~$n \in \omega$, some sequence of clopen sets~$V_0, \dots, V_{m-1} \subseteq 2^{=n}$ such that $\bigcap_{s < m} [V_s] = \emptyset$ and some~$k \in \omega$ such that, for every~$s < m$, the following class is non-empty:
\ludovic{No, we need to check that $(Y, V) \in \V$}
$$
\C_s = \left\{ Z_0 \oplus \dots \oplus Z_{k-1} : 
	\begin{array}{l}
		Z_0 \cup \dots \cup Z_{k-1} = \omega \wedge\\
		\forall i < k\ (Z_i, V_s) \not \in \V \vee \forall \rho \subseteq Z_i\ \Phi_e^{\sigma \cup \rho}(n)\uparrow \vee [\Phi_e^{\sigma \cup \rho}(n)] \cap [V_s] \neq \emptyset 
	\end{array} \right\}
%Z_0 \cup \dots \cup Z_{k-1} = \omega \wedge \forall i < k \forall \rho \subseteq Z_i\ \Phi_e^{\sigma \cup \rho}(n)\uparrow \vee [\Phi_e^{\sigma \cup \rho}(n)] \cap [V_s] \neq \emptyset  \}
$$
Note that $\C_s$ is a non-empty $\Pi^0_1$ class. Pick any element $Z^s_0 \oplus \dots \oplus Z^s_{k-1} \in \C_s$. By \Cref{lemma:prtrace-abslarge}, there is a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ subclass $\W$ of~$\U$ and some $(i_s < k : s < m)$ such that $Y = \bigcap_{s < m} Z^s_{i_s} \cap X$ is $\mathfrak{T}(\C)$-generic in $\W$. The condition $(\sigma, Y, \W)$ is an desired extension of~$(\sigma, X, \V)$ forcing $\Phi_e^{G}(n)\uparrow$.
\end{proof}

We are now ready to prove \Cref{thm:pg-traceg-ce}.
Let~$\F$ be a sufficiently generic filter containing $(\emptyset, A, \U)$. By \Cref{lem:pg-traceg-forcing-infinite}, $G_\F$ is infinite. By construction, $G_\F \subseteq A$. Last, by \Cref{lem:pg-traceg-forcing-requirement}, $B$ is not $\Sigma^0_1(G_\F)$.
\end{proof}


\begin{corollary}\label[corollary]{cor:non-ce-pg-closed-avoidance-nonce}
Let~$\C \subseteq 2^\omega$ be a closed class with no computable c.b-trace. Let~$A$ be partition generic relative to~$\C$. 
Then there is an infinite subset~$H \subseteq A$ such that~$\C$ has no $H$-computable c.b-trace.
\end{corollary}
\begin{proof}
By~\Cref{prop:nocb-and-pg-rel-then-prtrace-gen}, $A$ is $\mathfrak{T}(\C)$-generic.
By \Cref{thm:pg-traceg-ce}, there is an infinite subset~$H \subseteq A$ such that~$\C$ has no $H$-computable c.b-trace.
\end{proof}

\begin{corollary}
Let~$\C \subseteq 2^\omega$ be a closed class with no computable c.b-trace. Let~$A$ be Kurtz random relative to~$\C$.
Then there is an infinite subset~$H \subseteq A$ such that~$\C$ has no $H$-computable c.b-trace.
\end{corollary}
\begin{proof}
By \Cref{prop:kurtz-bipg}, $A$ is partition generic relative to~$\C$, so by \Cref{cor:non-ce-pg-closed-avoidance-nonce}, there is an infinite subset~$H \subseteq A$ such that~$\C$ has no $H$-computable c.b-trace.
\end{proof}

\begin{proof}[Proof of~\Cref{thm:avoidance-closed-pigeon-basis}]
Let~$\C \subseteq 2^\omega$ be a closed class with no computable c.b-trace, and $A$ be a set.
By \Cref{prop:prtrace-pg-omega-ce}, $\omega$ is $\mathfrak{T}(\C)$-generic.
By \Cref{lemma:prtrace-abslarge}, there is a non-trivial $\mathfrak{T}(\C)$-large $\Sigma^0_1$ class~$\A \subseteq 2^\omega \times \P(2^{<\omega})$ within which either~$A$ or $\overline{A}$ is $\mathfrak{T}(\C)$-generic. By \Cref{thm:pg-traceg-ce}, there is an infinite subset~$H \subseteq A$ such that~$\C$ has no $H$-computable c.b-trace.
\end{proof}

\ludovic{The previous theorem is false. There are closed sets~$\C \subseteq 2^\omega$ with no computable c.b-trace, but with a computable 2-trace. Then, given $(\sigma_n, \tau_n)_{n \in \omega}$ a computable 2-trace of~$\C$, let~$A = \{ n : [\sigma_n] \cap \C \neq \emptyset \}$. Every infinite subset of~$A$ or of~$\overline{A}$ compute an infinite c.b-trace of~$\C$.}




